Too Few Bug Reports? Exploring Data Augmentation for Improved Changeset-based Bug Localization

Modern Deep Learning (DL) architectures based on transformers (e.g., BERT, RoBERTa) are exhibiting performance improvements across a number of natural language tasks. While such DL models have shown tremendous potential for use in software engineering applications, they are often hampered by insufficient training data. Particularly constrained are applications that require project-specific data, such as bug localization, which aims at recommending code to fix a newly submitted bug report. Deep learning models for bug localization require a substantial training set of fixed bug reports, which are at a limited quantity even in popular and actively developed software projects. In this paper, we examine the effect of using synthetic training data on transformer-based DL models that perform a more complex variant of bug localization, which has the goal of retrieving bug-inducing changesets for each bug report. To generate high-quality synthetic data, we propose novel data augmentation operators that act on different constituent components of bug reports. We also describe a data balancing strategy that aims to create a corpus of augmented bug reports that better reflects the entire source code base, because existing bug reports used as training data usually reference a small part of the code base.

==> background.tex <==
% \section{Background and Related work}
\section{Related work}



\subsection{Bug localization with deep learning}
% explain this paper is about bug-inducing changesets
As an approach to mitigate the high cost of software maintenance, bug localization aims to help developers by automatically locating the program elements relevant to a bug described in a newly submitted bug report. Bug localization is a topic that has been of interest to researchers for a number of years with considerable progress being made by techniques like BugLocator~\cite{buglocator}, BugScout~\cite{bugscout} and BRTracer~\cite{wong_brtracer_2014}, which excel at retrieving program elements (i.e., methods, classes) for bug reports that contain terms that directly appear in the code base. 
However, recently researchers and practitioners have recognized two important modifications to the traditional formulation of bug localization:
%However, recently researchers have also been interested in two modifications to this topic: 
1) retrieving changesets that induced the bug instead of classes or methods, because they contain valuable information for developers 
%(e.g., description of the change provided in the log, name of a developer that introduced the change)
and may be easier to examine~\cite{wen2016,murali2020industry}; and 2) using deep learning techniques in order to go beyond simple string matching and capture semantic similarity between bug reports and code~\cite{huo2019deep}. 
Bug inducing changesets provide several conveniences to developers that are looking to fix a bug. They capture the lines of code that are related, in the context of a specific modification to the code. The modification is also described by the commit log message. Changesets also indicate the developer responsible for the change, which can facilitate fast bug triage. Finally, changesets can be decomposed into a set of hunks, i.e., a set of changes in one area of the file, which are usually straightforward to comprehend.

To achieve the goal of using semantic matching to retrieve changesets for a newly submitted bug report, of particular interest are Transformer-based architectures that can be pre-trained on a large corpus (e.g., BERT, RoBERTa). While fine tuning such models enables their application for problems where data is scarce, the models are typically trained on general corpora (e.g., Wikipedia), which may not reflect the specific patterns of software engineering data~\cite{gururangan2020don}. To address this problem, a few BERT models pre-trained on large-scale software engineering  data (e.g., GitHub, Stack Overflow) have been created~\cite{tabassum2020code,feng2020codebert}. 
Lin et al.~\cite{lin2021traceability} proposed to further improve the performance of transformer-based models by introducing an extra step called intermediate pre-training, which uses a large corpus of data that is closely related to the downstream task (i.e., code search) to continue pre-training the model. 
Another body of work concentrates on custom DL architectures that enable incorporating data from multiple software projects in training the model.
For instance, Huo et al.~\cite{huo2016learning} proposed using neural networks to learn a unified feature space for bug reports and source code that better reflects the correlation between the two types of documents. 
In their later work~\cite{huo2019deep}, this approach was revised to extract and train on features that are transferable between different projects (i.e., cross-project).
Zhu et al.~\cite{Zhu2020CooBaCB} proposed another cross-project bug localization technique that utilizes adversarial transfer learning.

\subsection{Data augmentation}
% Why DA?
% The success of deep learning is dependent upon leveraging large amount of labelled data, which, for many tasks and domains, is expensive and time-consuming to collect at scale.
% Data Augmentation (DA) is a recent strategy to alleviate this data scarcity issue.
% What is DA and how new samples are created
Data Augmentation (DA) aims to generate high quality, synthetic training examples from the already available data. 
To this end, DA transforms the existing training examples to create new data points that expand the original training set with the ultimate goal of improving the performance of the downstream DL model. DA was successfully adopted in the computer vision domain, where simple image transformations, such as rotation or color manipulation, allow for the creation of an abundance of new data points to train the model on, thus leading to significant improvements in image classification tasks~\cite{szegedy2015going, wong2016understanding}.


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.7\columnwidth]{figures/cv.pdf}
%     \caption{Example of data augmentation transformations in computer vision domain.}
%     \label{fig:cv}
% \end{figure}

% Although the general concept of DA is easy to grasp, i.e., generating new data from the existing training set, the question of {\em how to} is very domain- or task-specific.
% Given a dataset, performing DA requires answering the following questions: (1) what are the data transformations that can create synthetic training examples, and (2) how the quality of those examples can be assured. Depending on the problem, the answers to those questions vary. For instance, in image classification there exist multiple well-established methods to produce augmented data, examples of which are depicted in Figure~\ref{fig:cv}. 
% The key property of these transformations is that they are label invariant (i.e., a rotated or flipped image of dog, is still an image of a dog), which is fundamental to generating good quality labelled training examples.

Designing similar data transformations for textual data is significantly more challenging given the discrete nature of language. 
More specifically, compared to image transformations, augmenting textual data is more prone to inadvertently distorting the text's semantics, which in turn, can affect the original label. In other words, the transformation may not be label invariant. 
To prevent this from happening, researchers in NLP proposed numerous DA strategies ranging from simple rule-based techniques to transformations leveraging advanced DL models~\cite{shorten2021text,feng2021survey}. 

Rule-based techniques rely on data transformations that typically extend and re-arrange the existing data. 
For instance, Wei and Zou.~\cite{wei2019eda} proposed Easy Data Augmentation (EDA), which encompasses four token-level operators: random insert, random swap, random delete, and synonym replacement. The operators are applied only to a small portion of words (e.g., 1\%) to minimize the risk of affecting the label. EDA improves the performance of text classification tasks, with the highest boost observed for the smallest datasets (i.e., 500 samples). 
Sahin et al.~\cite{sahin2018data} introduced a sentence-level augmenter that uses a dependency tree to maintain the invariance of the sentence while swapping or deleting child nodes. 
Guided by in-domain knowledge, Yan et al.~\cite{yan2019data} proposed to randomly delete sentences in lengthy legal documents as many of them are irrelevant to the understanding of the case. The strength of rule-based techniques lies in the ease of use and interpretability of the augmentation operators, while the strict augmentation rules help to enforce label invariance.


This question of label preserving data transformations can be further extended to the overall question of quality and diversity of newly generated training examples.
%The question of label preserving data transformations can be further extended as, while a data transformation should be invariant with respect to the original label, it should also introduce some diversity to the training data. 
In other words, a synthetic example should be different enough from the original example to add ``new value`` to the training set, and similar enough to preserve the original label. 
Given that rule-based DA techniques follow a rigid and fixed set of rules, they have limited ability to produce diverse output.
To overcome that, another branch of DA methods use external models. For instance, Guo et al.~\cite{guo2019augmenting} uses embeddings to convert text to a numeric vector, and subsequently mixes pairs of numeric vectors to create synthetic examples. 
Backtranslation~\cite{sennrich2016improving,li2020diverse} is another popular method used to paraphrase the original data by translating a sentence to another language and back~\cite{kumar2019submodular,xie2020unsupervised,fabbri2021improving}. More recently, researchers explored generative data augmentation with the help of pre-trained GPT-2 models~\cite{anaby2020not,quteineh2020textual}. While these methods are able to extrapolate further from the existing data, and, hence lead to more diverse augmentation, they require a good quality pre-trained models and are computationally expensive~\cite{feng_learn2augment_2021}. Moreover, the recent work of Kovatchev et al.~\cite{kovatchev2021vectors} points out that for domain-specific tasks, DA using models pre-trained on out-of-domain data, can be in fact outperformed by carefully designed rule-based operators that take into account a dictionary specific to the task. Interestingly, the authors reported to achieve the best performance when combining multiple, simple data transformations to generate a new example. While combining data transformations, known as stacking augmentations~\cite{shorten2021text}, is often used in the computer vision domain, it has only recently been effectively applied to textual data~\cite{kovatchev2021vectors, qu2020coda}. 

%Applying DA bring also a several other practical considerations related to the strength of the augmentation.

%Ding et al.~\cite{ding2020daga} propose an LSTM model to generate new context for a selected token. 

%Note that while it is acceptable for DA to introduce a small amount of noise when augmenting data, since it makes the model more robust to the noise in general, the number of poor quality examples or invalid examples should be kept low.


%In general, data augmentation (DA) increases the training set size by generating new, synthetic training data with the ultimate goal of improving the performance of the downstream model. To this end, DA uses the already available training set, possibly small, and modifies
%The main goal of data augmentation is to create new, synthetic data from the existing training data, 
%The main goal of data augmentation (DA) is to increase the size of the training set for problems that experience labelled data scarcity.

%How new samples are created (in general)
%To this end, DA techniques create new, synthetic examples by applying various transformations to the available data, such that the newly constructed data (i.e., the augmented data) preserves the initial label and remains valid for the task, i.e., the key characteristics of the original data remains intact~\cite{raille2020fast}. 
%As an example, consider simple image transformations depicted in Figure~\ref{fig:cv}, that are commonly used to augment data in the computer vision domain~\cite{szegedy2015going}. Each transformation produce slightly modified image, yet preserves the label (i.e., a dog is still a dog), and the key characteristics (e.g., shape of the animal). 


% DA in NLP: challenges, approaches, types
%Designing similar data transformations for the text domain is significantly more challenging given the discrete nature of language. Augmenting textual data is susceptible to inadvertently distorting the text and invalidating its semantics, which, in turn, can affect the original labels. To account for the quality of textual augmentation, researchers in NLP explored different approaches ranging from rule-based techniques to methods leveraging advanced DL models~\cite{shorten2021text,feng2021survey}, and each category provides its own set of trade offs. Rule-based techniques relies on operators that typically extend and re-arrange the existing data. For instance, Wei and Zou.~\cite{wei2019eda} proposed Easy Data Augmentation (EDA) that encompass four token-level operators: random insert, random swap, random delete, and synonym replacement. While EDA improves the performance on text classification task, the highest gain is observed for the smallest dataset (i.e., 500 samples). Sahin et al.~\cite{sahin2018data} introduced a sentence-level augmenter that uses a dependency tree to maintain invariance of the sentence while swapping or deleting children nodes. Guided by in-domain knowledge, Yan et al.~\cite{yan2019data} proposed to randomly delete sentences in lengthy legal documents as many of them are irrelevant to the understanding of the case. The strength of rule-based techniques lies in the ease of use and interpretability of the augmentation operators, often driven by domain expertise. However, the control over the augmentation process given by rule-based methods comes at a price of less diverse output of the augmentation. To overcome that, another branch of DA methods use external models. For instance, Guo et al.~\cite{guo2019augmenting} uses embeddings to represent text as numeric vectors that can be interpolated to create more diverse data. Backtranslation method~\cite{sennrich2016improving,li2020diverse} can be used to translate a sentence to another language and back to its original language to create paraphrases of the original data~\cite{kumar2019submodular,xie2020unsupervised,fabbri2021improving}. Most recently, researchers explored generative data augmentation which aims to generate new data with the help of pre-trained GPT-2 models~\cite{anaby2020not,quteineh2020textual}. While those methods are able to extrapolate further from the existing data, and, hence lead to more diverse augmentation, they require a good quality pre-trained models, and are significantly more computationally expensive.


%While the primary goal of DA is to increase the size of the training set for tasks experiencing data scarcity~\cite{fadaee2017data,li2020diverse}, augmenting the data brings a few other benefits over the original datasets. First, using augmented data helps in preventing overfitting to the training data. Secondly, the augmented data can be used to fix the data distribution in case of data imbalance~\cite{lee2021neural,wei2021few,kumar2019closer}. 




==> big_table.tex <==
\appendices

\section{Results per project}
\label{ap:results-per-project}

\begin{table*}[]
\centering
\scriptsize
\begin{tabular}{l|lllll|lllll|lllll}
\toprule
 & \textbf{MRR} & \textbf{MAP} & \textbf{P@1} & \textbf{P@3} & \textbf{P@5} & \textbf{MRR} & \textbf{MAP} & \textbf{P@1} & \textbf{P@3} & \textbf{P@5} & \textbf{MRR} & \textbf{MAP} & \textbf{P@1} & \textbf{P@3} & \textbf{P@5} \\ \midrule
 & \multicolumn{5}{c}{\textbf{FBL-BERT}} & \multicolumn{5}{c}{\textbf{TBERT-Siamese}} & \multicolumn{5}{c}{\textbf{TBERT-Single}} \\ \midrule \midrule
 & \multicolumn{15}{c}{\textit{All (\# bug reports = 331)}} \\ \midrule
$D_{ori}$ & 0.264          & 0.109          & 0.163          & 0.153          & 0.145          & 0.180          & 0.062          & 0.144          & 0.076          & 0.069          & 0.273          & 0.120          & 0.162 & 0.145 & 0.149 \\
$D_{rep}$ & 0.307\textsuperscript{$\uparrow$} & 0.129\textsuperscript{$\uparrow$} & 0.213\textsuperscript{$\uparrow$} & 0.179          & 0.176          & 0.201          & 0.086          & 0.110          & 0.093          & 0.093          & 0.271          & 0.140\textsuperscript{$\uparrow$} & 0.152 & 0.136\textsuperscript{$\uparrow$} & 0.176 \\
$D_{aug}$ & 0.353\textsuperscript{$\uparrow$} & 0.146\textsuperscript{$\uparrow$} & 0.247\textsuperscript{$\uparrow$} & 0.202\textsuperscript{$\uparrow$} & 0.197\textsuperscript{$\uparrow$} & 0.236          & 0.103          & 0.157          & 0.124          & 0.119\textsuperscript{$\uparrow$} & 0.333\textsuperscript{$\uparrow$} & 0.144\textsuperscript{$\uparrow$} & 0.217\textsuperscript{$\uparrow$} & 0.188\textsuperscript{$\uparrow$} & 0.194\textsuperscript{$\uparrow$} \\
$D_{bl*}$ & 0.367\textsuperscript{$\uparrow$} & 0.147\textsuperscript{$\uparrow$} & 0.267\textsuperscript{$\uparrow$} & 0.198\textsuperscript{$\uparrow$} & 0.206\textsuperscript{$\uparrow$} & 0.328\textsuperscript{$\uparrow$} & 0.107\textsuperscript{$\uparrow$} & 0.247\textsuperscript{$\uparrow$} & 0.150\textsuperscript{$\uparrow$} & 0.146\textsuperscript{$\uparrow$} & 0.368\textsuperscript{$\uparrow$} & 0.149\textsuperscript{$\uparrow$} & 0.269\textsuperscript{$\uparrow$} & 0.192\textsuperscript{$\uparrow$} & 0.182\textsuperscript{$\uparrow$} \\  \midrule 
 & \multicolumn{15}{c}{\textit{Aspectj (\# bug reports = 100)}} \\ \midrule
$D_{ori}$ & 0.122          & 0.064          & 0.051          & 0.074          & 0.085          & 0.193          & 0.094 & 0.175 & 0.091 & 0.091 & 0.148          & 0.065          & 0.050 & 0.058 & 0.103 \\
$D_{rep}$ & 0.146          & 0.082          & 0.072          & 0.089          & 0.114          & 0.145          & 0.082 & 0.082 & 0.084 & 0.085 & 0.201\textsuperscript{$\uparrow$} & 0.108\textsuperscript{$\uparrow$} & 0.120\textsuperscript{$\uparrow$} & 0.092 & 0.167 \\
$D_{aug}$ & 0.215\textsuperscript{$\uparrow$} & 0.118\textsuperscript{$\uparrow$} & 0.134\textsuperscript{$\uparrow$} & 0.144\textsuperscript{$\uparrow$} & 0.154\textsuperscript{$\uparrow$} & 0.208\textsuperscript{$\uparrow$} & 0.104 & 0.165 & 0.106 & 0.107 & 0.194\textsuperscript{$\uparrow$} & 0.110\textsuperscript{$\uparrow$} & 0.110\textsuperscript{$\uparrow$} & 0.113\textsuperscript{$\uparrow$} & 0.138 \\
$D_{bl*}$ & 0.206\textsuperscript{$\uparrow$} & 0.113\textsuperscript{$\uparrow$} & 0.123\textsuperscript{$\uparrow$} & 0.134\textsuperscript{$\uparrow$} & 0.179\textsuperscript{$\uparrow$} & 0.193          & 0.096 & 0.165 & 0.094 & 0.109 & 0.194\textsuperscript{$\uparrow$} & 0.100\textsuperscript{$\uparrow$} & 0.130\textsuperscript{$\uparrow$} &0.102\textsuperscript{$\uparrow$} & 0.108 \\ \midrule
 & \multicolumn{15}{c}{\textit{SWT (\# bug reports = 45)}} \\ \midrule
$D_{ori}$ & 0.473          & 0.168 & 0.398 & 0.245 & 0.199 & 0.535 & 0.136          & 0.498 & 0.224 & 0.180 & 0.424          & 0.186 & 0.411 & 0.270 & 0.238 \\
$D_{rep}$ & 0.384          & 0.159 & 0.249 & 0.241 & 0.228 & 0.500 & 0.163          & 0.348 & 0.245 & 0.230\textsuperscript{$\uparrow$} & 0.302\textsuperscript{$\uparrow$} & 0.132 & 0.145\textsuperscript{$\uparrow$} & 0.133\textsuperscript{$\uparrow$} & 0.189\textsuperscript{$\uparrow$} \\
$D_{aug}$ & 0.408          & 0.152 & 0.299 & 0.212 & 0.196 & 0.423 & 0.186\textsuperscript{$\uparrow$} & 0.249 & 0.282 & 0.243\textsuperscript{$\uparrow$} & 0.391          & 0.152 & 0.242 & 0.231 & 0.202 \\
$D_{bl*}$ & 0.595\textsuperscript{$\uparrow$} & 0.196 & 0.498 & 0.290 & 0.271 & 0.607 & 0.189\textsuperscript{$\uparrow$} & 0.523 & 0.299\textsuperscript{$\uparrow$} & 0.255\textsuperscript{$\uparrow$} & 0.435\textsuperscript{$\uparrow$} & 0.171 & 0.290 & 0.251 & 0.219 \\ \midrule
 & \multicolumn{15}{c}{\textit{Tomcat (\# bug reports = 97)}} \\ \midrule
$D_{ori}$ & 0.318          & 0.144          & 0.210          & 0.197          & 0.180          & 0.083         & 0.030          & 0.044          & 0.037          & 0.036          & 0.358          & 0.182          & 0.193 & 0.213 & 0.209 \\
$D_{rep}$ & 0.462\textsuperscript{$\uparrow$} & 0.195\textsuperscript{$\uparrow$} & 0.353\textsuperscript{$\uparrow$} & 0.276\textsuperscript{$\uparrow$} & \textbf{0.25}2 &0.187\textsuperscript{$\uparrow$} & 0.094\textsuperscript{$\uparrow$} & 0.088          & 0.079          & 0.084          & 0.371          & 0.208          & 0.236 & 0.209 & 0.216 \\
$D_{aug}$ & 0.450\textsuperscript{$\uparrow$} & 0.187\textsuperscript{$\uparrow$} & 0.342\textsuperscript{$\uparrow$} & 0.257\textsuperscript{$\uparrow$} & 0.235\textsuperscript{$\uparrow$} &0.251\textsuperscript{$\uparrow$} & 0.121\textsuperscript{$\uparrow$} & 0.165          & 0.129\textsuperscript{$\uparrow$} & 0.132\textsuperscript{$\uparrow$} & 0.493\textsuperscript{$\uparrow$} & 0.207          & 0.374\textsuperscript{$\uparrow$} & 0.278\textsuperscript{$\uparrow$} & 0.278\textsuperscript{$\uparrow$} \\
$D_{bl*}$ & 0.452\textsuperscript{$\uparrow$} & 0.193\textsuperscript{$\uparrow$} & 0.342\textsuperscript{$\uparrow$} & 0.259\textsuperscript{$\uparrow$} & 0.237\textsuperscript{$\uparrow$} &0.474\textsuperscript{$\uparrow$} & 0.133\textsuperscript{$\uparrow$} & 0.364\textsuperscript{$\uparrow$} & 0.206\textsuperscript{$\uparrow$} & 0.199\textsuperscript{$\uparrow$} & 0.578\textsuperscript{$\uparrow$} & 0.217\textsuperscript{$\uparrow$} & 0.452\textsuperscript{$\uparrow$} & 0.296\textsuperscript{$\uparrow$} & 0.260\textsuperscript{$\uparrow$} \\ \midrule
 & \multicolumn{15}{c}{\textit{PDE (\# bug reports = 30)}} \\ \midrule
$D_{ori}$ & 0.243          & 0.089 & 0.143          & 0.101          & 0.122          & 0.073          & 0.015          & 0.036 & 0.012 & 0.014          & 0.228          & 0.077          & 0.104 & 0.087 & 0.081 \\
$D_{rep}$ & 0.352          & 0.135 & 0.285          & 0.196          & 0.149          & 0.078          & 0.050          & 0.000 & 0.012 & 0.040          & 0.289          & 0.177\textsuperscript{$\uparrow$} & 0.139\textsuperscript{$\uparrow$} & 0.179\textsuperscript{$\uparrow$} & 0.221\textsuperscript{$\uparrow$} \\
$D_{aug}$ & 0.422\textsuperscript{$\uparrow$} & 0.160 & 0.357\textsuperscript{$\uparrow$} & 0.214\textsuperscript{$\uparrow$} & 0.204          & 0.119          & 0.032          & 0.071 & 0.048 & 0.037          & 0.363\textsuperscript{$\uparrow$} & 0.165\textsuperscript{$\uparrow$} & 0.243\textsuperscript{$\uparrow$} & 0.214\textsuperscript{$\uparrow$} & \textbf{
0.219} \\
$D_{bl*}$ & 0.400\textsuperscript{$\uparrow$} & 0.163 & 0.285\textsuperscript{$\uparrow$} & 0.196          & 0.234\textsuperscript{$\uparrow$} & 0.130\textsuperscript{$\uparrow$} & 0.042\textsuperscript{$\uparrow$} & 0.036 & 0.059 & 0.062\textsuperscript{$\uparrow$} & 0.407\textsuperscript{$\uparrow$} & 0.201\textsuperscript{$\uparrow$} & 0.312\textsuperscript{$\uparrow$} & 0.238\textsuperscript{$\uparrow$} & 0.265\textsuperscript{$\uparrow$} \\ \midrule
 & \multicolumn{15}{c}{\textit{JDT (\# bug reports = 47)}} \\ \midrule
$D_{ori}$ & 0.288 & 0.095 & 0.114 & 0.186 & 0.169 & 0.094          & 0.017          & 0.023 & 0.030 & 0.023          & 0.267 & 0.081          & 0.155 & 0.118 & 0.091 \\
$D_{rep}$ & 0.245 & 0.064 & 0.159 & 0.114 & 0.126 & 0.156          & 0.031          & 0.068 & 0.053 & 0.039          & 0.176 & 0.051\textsuperscript{$\uparrow$} & 0.066 & 0.059 & 0.072 \\
$D_{aug}$ & 0.360 & 0.105 & 0.182 & 0.197 & 0.209 & 0.167          & 0.033          & 0.091 & 0.053 & 0.053\textsuperscript{$\uparrow$} & 0.231 & 0.062          & 0.089 & 0.103 & 0.114 \\
$D_{bl*}$ & 0.319 & 0.075 & 0.205 & 0.129 & 0.124 & 0.193\textsuperscript{$\uparrow$} & 0.043\textsuperscript{$\uparrow$} & 0.068 & 0.076 & 0.071\textsuperscript{$\uparrow$} & 0.283 & 0.063          & 0.155 & 0.100 & 0.098 
\\ \bottomrule
\end{tabular}
\end{table*}


==> biography.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}{Michael Shell}
Biography text here.
\end{IEEEbiography}

% if you will not have a photo at all:
\begin{IEEEbiographynophoto}{John Doe}
Biography text here.
\end{IEEEbiographynophoto}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

\begin{IEEEbiographynophoto}{Jane Doe}
Biography text here.
\end{IEEEbiographynophoto}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}
